The Cosmological Parameters (2021)

This is a review article for The Review of Particle Physics 2022 (aka the Particle Data Book). It forms a compact review of knowledge of the cosmological parameters near the end of 2021. Topics included are Parametrizing the Universe; Extensions to the standard model; Probes; Bringing observations together; Outlook for the future.

==> pdgdefs.tex <==
% $Id: pdgdefs.tex 27857 2020-07-08 00:40:21Z beringer $
% Definition of standard PDG macros for reviews
%
% ------------------------------------------------
% DO NOT EDIT THIS FILE - ALL CHANGES WILL BE LOST
%
% If you wish to update the PDG definitions, please
% update ProdTools/reviewtemplate/pdgdefs.tex.
% ------------------------------------------------

%
% RPP definitions
%
\def\journalNameBrief{~}
\def\pubVol{~}        % publication volume
\def\pubArticleId{~}
\def\pubPageId{\pubArticleId}	% alternate formats used in citation
\def\pubPage{~}            % publication page
\def\pubYear{2022}	% current publication year
\def\JournalVol{\journalNameBrief\ {\bf \pubVol}, \pubPageId\ (\pubYear)}
\def\primaryAuthor{In The Review of Particle Physics}% 2020
\def\rppCitation{\primaryAuthor, Particle Data Group (2022)}
\def\rppCitationSumTab{Particle Data Group}
\def\rppDOI{~}

%
% Funding agencies
%
\def\DOEnumber{DE--AC02--05CH11231}  
\def\pdgfunding{The publication of the {\sl Review of Particle Physics} is supported
by the Director, Office of Science, Office of High Energy Physics of the U.S. Department of Energy under Contract No.\ \DOEnumber;
by the European Laboratory for Particle Physics (CERN); 
by an implementing arrangement between the governments of Japan (MEXT: Ministry of Education, Culture, Sports, Science and Technology) and the United States (DOE) on cooperative research and development; 
by the Italian National Institute of Nuclear Physics (INFN);
and by the Physical Society of Japan (JPS).
Individual collaborators receive support for their PDG activities from their respective funding agencies.}


%
% Utility macros
%
\def\Widebar#1{\vbox to 0pt{\vss\hbox{$\overline #1$}}}
\newcommand{\showsymbol}[1]{ 
  \texttt{\string#1} & #1 }
%\def\vec#1{\mathbfit{#1}}

%
% General definitions
%
\newcommand{\eg}{\mbox{\itshape e.g.}\xspace}
\newcommand{\ie}{\mbox{\itshape i.e.}\xspace}
\newcommand{\etal}{\mbox{\itshape et al.}\xspace}
\newcommand{\etc}{\mbox{\itshape etc.}\xspace}
\newcommand{\cf}{\mbox{\itshape cf.}\xspace}
\newcommand{\ffp}{\mbox{\itshape ff.}\xspace}
\newcommand{\vs}{\mbox{\itshape vs.}\xspace}
% TODO: the following needs to be checked by Piotr
\def\ibid{{\it ibid.}}
\def\Ref#1{Ref.~\cite{#1}}
\newcommand{\Tab}[1]{Table~\ref{#1}}
\newcommand{\Section}[1]{Section~\ref{#1}}
\newcommand{\Sec}[1]{Sec.~\ref{#1}}
\newcommand{\Figure}[1]{Figure~\ref{#1}}
\newcommand{\Fig}[1]{Fig.~\ref{#1}}
\def\Eq#1{Eq.~(\ref{#1})}
\newcommand{\gsim}{\gtrsim}   % requires amssymb
\newcommand{\lsim}{\lesssim}  % requires amssymb

%
% Energy and momentum
%
\newcommand*{\TeV}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand*{\GeV}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand*{\MeV}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand*{\keV}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand*{\meV}{\ensuremath{\mathrm{\,me\kern -0.1em V}}\xspace}
\newcommand*{\eV  }{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand*{\GeVc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand*{\GeVcSq}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V^2\!/}c^2}}\xspace}
\newcommand*{\GeVcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand*{\GeVccSq}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V^2\!/}c^4}}\xspace}
\newcommand*{\MeVc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand*{\MeVcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}

%
% Distance
%
\newcommand*{\syin }{\ensuremath{^{\prime\prime}}\xspace}                 
\newcommand*{\inch }{\ensuremath{\rm \,in}\xspace} % \in is taken	 
\newcommand*{\ft   }{\ensuremath{\rm \,ft}\xspace}			 
\newcommand*{\km   }{\ensuremath{{\rm \,km}}\xspace}			 
\newcommand*{\m    }{\ensuremath{{\rm \,m}}\xspace}			 
\newcommand*{\cm   }{\ensuremath{{\rm \,cm}}\xspace}			 
\newcommand*{\mm   }{\ensuremath{{\rm \,mm}}\xspace}			 
\newcommand*{\mum  }{\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter 	 
\newcommand*{\nm   }{\ensuremath{{\rm \,nm}}\xspace}			 
\newcommand*{\fm   }{\ensuremath{{\rm \,fm}}\xspace}			 

%
% Area
%
\def\ma  {\ensuremath{{\rm \,m}^2}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
\def\muma {\ensuremath{{\,\mu\rm m}^2}\xspace}

%
% Cross-section
%
\def\barn      {\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph  {\ensuremath{{\rm -b}}\xspace}
\def\mbarn     {\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph {\ensuremath{{\rm -mb}}\xspace}
\def\microbarn {\ensuremath{\,\mu{\rm b}}\xspace}
\def\nb        {\ensuremath{{\rm \,nb}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}

%
% Luminosity
%
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}

%
% Frequency
%
\def\invps {\ensuremath{\mbox{\,ps}^{-1}}\xspace}


%
% Miscellaneous
%
\newcommand{\lum}     {\ensuremath{\mathcal{L}}\xspace}
\newcommand{\chisq}   {\ensuremath{\chi^2}\xspace}
\newcommand*{\degr}    {\ensuremath{^\circ}}

%
% Particles
%

% +--------------------------------------------------------------------+
% |  Particle-antiparticle pair notations                              |
% +--------------------------------------------------------------------+
\newcommand*{\pp}{\ensuremath{pp}\xspace}
\newcommand*{\antibar}[1]{\ensuremath{#1\bar{#1}}\xspace}
\newcommand*{\pbar}{\ensuremath{\bar{p}}\xspace}
\newcommand*{\ppbar}{\antibar{p}}
\newcommand*{\tbar}{\ensuremath{\bar{t}}\xspace}
\newcommand*{\ttbar}{\antibar{t}}
\newcommand*{\bbar}{\ensuremath{\bar{b}}\xspace}
\newcommand*{\bbbar}{\antibar{b}}
\newcommand*{\cbar}{\ensuremath{\bar{c}}\xspace}
\newcommand*{\ccbar}{\antibar{c}}
\newcommand*{\sbar}{\ensuremath{\bar{s}}\xspace}
\newcommand*{\ssbar}{\antibar{s}}
\newcommand*{\ubar}{\ensuremath{\bar{u}}\xspace}
\newcommand*{\uubar}{\antibar{u}}
\newcommand*{\dbar}{\ensuremath{\bar{d}}\xspace}
\newcommand*{\ddbar}{\antibar{d}}
\newcommand*{\fbar}{\ensuremath{\bar{f}}\xspace}
\newcommand*{\ffbar}{\antibar{f}}
\newcommand*{\qbar}{\ensuremath{\bar{q}}\xspace}
\newcommand*{\qqbar}{\antibar{q}}
\newcommand*{\nbar}{\ensuremath{\bar{\nu}}\xspace}
\newcommand*{\nnbar}{\antibar{\nu}}

\newcommand*{\neutron}{\ensuremath{n}\xspace}
\newcommand*{\antineutron}{\ensuremath{\bar {n}}\xspace}
\newcommand*{\deuteron}{\ensuremath{d}\xspace}

% +--------------------------------------------------------------------+
% |  e+e-, etc.                                                        |
% +--------------------------------------------------------------------+
\newcommand*{\ee}{\ensuremath{e^{+} e^{-}}\xspace}
\newcommand*{\epm}{\ensuremath{e^{\pm}}\xspace}
\newcommand*{\epem}{\ensuremath{e^{+} e^-}\xspace}

\newcommand*{\en}{\ensuremath{e^{-}}\xspace} 
\newcommand*{\ep}{\ensuremath{e^{+}}\xspace}

\newcommand*{\mumu}{\ensuremath{\mu^{+} \mu^{-}}\xspace}
\newcommand*{\mun}{\ensuremath{\mu^{-}}\xspace}
\newcommand*{\mup}{\ensuremath{\mu^{+}}\xspace}

\newcommand*{\tautau}{\ensuremath{\tau^{+} \tau^{-}}\xspace}
\newcommand*{\taup}{\ensuremath{\tau^{+}}\xspace}
\newcommand*{\taum}{\ensuremath{\tau^{-}}\xspace}

\newcommand*{\lepton}{\ensuremath{\ell}\xspace}
\newcommand*{\leptonm}{\ensuremath{\ell^{-}}\xspace}
\newcommand*{\leptonp}{\ensuremath{\ell^{+}}\xspace}
\newcommand*{\leptonlepton}{\ensuremath{\ell^{+} \ell^{-}}\xspace}
\newcommand*{\ellell}{\ensuremath{\ell^{+} \ell^{-}}\xspace}
\newcommand*{\ellm}{\ensuremath{\ell^{-}}\xspace}
\newcommand*{\ellp}{\ensuremath{\ell^{+}}\xspace}

\newcommand*{\enu}{\ensuremath{e \nu}\xspace}
\newcommand*{\munu}{\ensuremath{\mu \nu}\xspace}
\newcommand*{\taunu}{\ensuremath{\tau \nu}\xspace}
\newcommand*{\lnu}{\ensuremath{\ell \nu}\xspace}


\newcommand*{\nub}        {\ensuremath{\bar{\nu}}\xspace}
\newcommand*{\nunub}{\antibar{\nu}}
\newcommand*{\nue}        {\ensuremath{\nu_{e}}\xspace}
\newcommand*{\nueb}       {\ensuremath{\nub_{e}}\xspace}
\newcommand*{\nuenueb}    {\ensuremath{\nue\nueb}\xspace}
\newcommand*{\num}        {\ensuremath{\nu_{\mu}}\xspace}
\newcommand*{\numb}       {\ensuremath{\nub_{\mu}}\xspace}
\newcommand*{\numnumb}    {\ensuremath{\num\numb}\xspace}
\newcommand*{\nut}        {\ensuremath{\nu_{\tau}}\xspace}
\newcommand*{\nutb}       {\ensuremath{\nub_{\tau}}\xspace}
\newcommand*{\nutnutb}    {\ensuremath{\nut\nutb}\xspace}

% +--------------------------------------------------------------------+
% |  Vector bosons                                                     |
% +--------------------------------------------------------------------+
\newcommand*{\Zzero}{\ensuremath{Z}\xspace}
\newcommand*{\Zboson}{\ensuremath{Z}\xspace}
\newcommand*{\Wplus}{\ensuremath{W^{+}}\xspace}
\newcommand*{\Wminus}{\ensuremath{W^{-}}\xspace}
\newcommand*{\Wboson}{\ensuremath{W}\xspace}
\newcommand*{\Wpm}{\ensuremath{W^{\pm}}\xspace}
\newcommand*{\Wmp}{\ensuremath{W^{\mp}}\xspace}

% +--------------------------------------------------------------------+
% |  pi, pi0, pi+, pi-, pi+-, eta, eta1, etc.                          |
% +--------------------------------------------------------------------+
\newcommand*{\pizero}{\ensuremath{\pi^{0}}\xspace}
\newcommand*{\piplus}{\ensuremath{\pi^{+}}\xspace}
\newcommand*{\piminus}{\ensuremath{\pi^{-}}\xspace}
\newcommand*{\pipm}{\ensuremath{\pi^{\pm}}\xspace}
\newcommand*{\pimp}{\ensuremath{\pi^{\mp}}\xspace}
\newcommand*{\etaprime}{\ensuremath{\eta^{\scriptscriptstyle\prime}}\xspace}

% +--------------------------------------------------------------------+
% |  K0, K+, K-, K0L, K0S                                              |
% +--------------------------------------------------------------------+
\def\Kbar{\mbox{\Widebar K}}
\newcommand*{\Kzero}{\ensuremath{K^{0}}\xspace}
\newcommand*{\Kzerobar}{\ensuremath{\overline{K}\vphantom{K}^{0}}\xspace}
\newcommand*{\kaon}{\ensuremath{K}\xspace}
\newcommand*{\Kplus}{\ensuremath{K^{+}}\xspace}
\newcommand*{\Kminus}{\ensuremath{K^{-}}\xspace}
\newcommand*{\KzeroL}{\ensuremath{K^{0}_{\text{L}}}\xspace}
\newcommand*{\Kzerol}{\ensuremath{K^{0}_{\text{L}}}\xspace}
\newcommand*{\Klong}{\ensuremath{K^{0}_{\text{L}}}\xspace}
\newcommand*{\KzeroS}{\ensuremath{K^{0}_{\text{S}}}\xspace}
\newcommand*{\Kzeros}{\ensuremath{K^{0}_{\text{S}}}\xspace}
\newcommand*{\Kshort}{\ensuremath{K^{0}_{\text{S}}}\xspace}
\newcommand*{\Kstar}{\ensuremath{K^{*}}\xspace}

% +--------------------------------------------------------------------+
% |  J/psi, psi prime, etc.                                            |
% +--------------------------------------------------------------------+
\newcommand*{\jpsi}{\ensuremath{J/\psi}\xspace}
\newcommand*{\Jpsi}{\ensuremath{J/\psi}\xspace}
\newcommand*{\psip}{\ensuremath{\psi(\text{2S})}\xspace}
\newcommand*{\chic}{\ensuremath{\raise.4ex\hbox{$\chi$}_{{c}}}\xspace}

% +--------------------------------------------------------------------+
% |                                                                    |
% |  Upsilons of various sorts                                         |
% |                                                                    |
% +--------------------------------------------------------------------+
\newcommand*{\UoneS}{\ensuremath{\mit\Upsilon(\text{1S})}\xspace}
\newcommand*{\Ups}[1]{\ensuremath{\mit{\Upsilon}(\text{#1S})}\xspace}
\newcommand*{\chib}{\ensuremath{\raise.4ex\hbox{$\chi$}_{{b}}}\xspace}

% +--------------------------------------------------------------------+
% |  C physics                                                         |
% +--------------------------------------------------------------------+
\newcommand*{\Dstar}{\ensuremath{D^{*}}\xspace}

% +--------------------------------------------------------------------+
% |  B physics                                                         |
% +--------------------------------------------------------------------+
\newcommand*{\Bd}{\ensuremath{B_{d}^{0}}\xspace}
\newcommand*{\Bs}{\ensuremath{B_{s}^{0}}\xspace}
\newcommand*{\Bu}{\ensuremath{B_{u}}\xspace}
\newcommand*{\Bc}{\ensuremath{B_{c}}\xspace}
\newcommand*{\Lb}{\ensuremath{\Lambda_{b}}\xspace}
\newcommand*{\Bstar}{\ensuremath{B^{*}}\xspace}
\newcommand*{\BoBo}{\ensuremath{B^{0}\mbox{--}\overline{B}^{0}}\xspace}
\newcommand*{\BodBod}{\ensuremath{B^{0}_{d}\mbox{--}\overline{B}^{0}_{d}}\xspace}
\newcommand*{\BosBos}{\ensuremath{B^{0}_{s}\mbox{--}\overline{B}^{0}_{s}}\xspace}

\newcommand*{\LambdaStar}{\ensuremath{\Lambda^{*}}}


% +--------------------------------------------------------------------+
% |                                                                    |
% | Hypothetical particles                                             |
% |                                                                    |
% +--------------------------------------------------------------------+
\newcommand*{\Azero }{\ensuremath{A^0}\xspace}
\newcommand*{\hzero }{\ensuremath{h^0}\xspace}
\newcommand*{\Hzero }{\ensuremath{H^0}\xspace}
\newcommand*{\Hboson}{\ensuremath{H}\xspace}
\newcommand*{\Hplus }{\ensuremath{H^+}\xspace}
\newcommand*{\Hminus}{\ensuremath{H^-}\xspace}
\newcommand*{\Hpm   }{\ensuremath{H^{\pm}}\xspace}
\newcommand*{\Hmp   }{\ensuremath{H^{\mp}}\xspace}
\newcommand*{\susy}[1]{\ensuremath{\tilde{#1}}\xspace}
\newcommand*{\ggino}{\ensuremath{\mathchoice%
      {\displaystyle\raise.4ex\hbox{$\displaystyle\tilde\chi$}}%
         {\textstyle\raise.4ex\hbox{$\textstyle\tilde\chi$}}%
       {\scriptstyle\raise.3ex\hbox{$\scriptstyle\tilde\chi$}}%
 {\scriptscriptstyle\raise.3ex\hbox{$\scriptscriptstyle\tilde\chi$}}}\xspace}

\newcommand*{\chinop}{\ensuremath{\mathchoice%
      {\displaystyle\raise.4ex\hbox{$\displaystyle\tilde\chi^+$}}%
         {\textstyle\raise.4ex\hbox{$\textstyle\tilde\chi^+$}}%
       {\scriptstyle\raise.3ex\hbox{$\scriptstyle\tilde\chi^+$}}%
 {\scriptscriptstyle\raise.3ex\hbox{$\scriptscriptstyle\tilde\chi^+$}}}\xspace}
\newcommand*{\chinom}{\ensuremath{\mathchoice%
      {\displaystyle\raise.4ex\hbox{$\displaystyle\tilde\chi^-$}}%
         {\textstyle\raise.4ex\hbox{$\textstyle\tilde\chi^-$}}%
       {\scriptstyle\raise.3ex\hbox{$\scriptstyle\tilde\chi^-$}}%
 {\scriptscriptstyle\raise.3ex\hbox{$\scriptscriptstyle\tilde\chi^-$}}}\xspace}
\newcommand*{\chinopm}{\ensuremath{\mathchoice%
      {\displaystyle\raise.4ex\hbox{$\displaystyle\tilde\chi^\pm$}}%
         {\textstyle\raise.4ex\hbox{$\textstyle\tilde\chi^\pm$}}%
       {\scriptstyle\raise.3ex\hbox{$\scriptstyle\tilde\chi^\pm$}}%
 {\scriptscriptstyle\raise.3ex\hbox{$\scriptscriptstyle\tilde\chi^\pm$}}}\xspace}
\newcommand*{\chinomp}{\ensuremath{\mathchoice%
      {\displaystyle\raise.4ex\hbox{$\displaystyle\tilde\chi^\mp$}}%
         {\textstyle\raise.4ex\hbox{$\textstyle\tilde\chi^\mp$}}%
       {\scriptstyle\raise.3ex\hbox{$\scriptstyle\tilde\chi^\mp$}}%
 {\scriptscriptstyle\raise.3ex\hbox{$\scriptscriptstyle\tilde\chi^\mp$}}}\xspace}

\newcommand*{\chinoonep}{\ensuremath{\mathchoice%
      {\displaystyle\raise.4ex\hbox{$\displaystyle\tilde\chi^+_1$}}%
         {\textstyle\raise.4ex\hbox{$\textstyle\tilde\chi^+_1$}}%
       {\scriptstyle\raise.3ex\hbox{$\scriptstyle\tilde\chi^+_1$}}%
 {\scriptscriptstyle\raise.3ex\hbox{$\scriptscriptstyle\tilde\chi^+_1$}}}\xspace}
\newcommand*{\chinoonem}{\ensuremath{\mathchoice%
      {\displaystyle\raise.4ex\hbox{$\displaystyle\tilde\chi^-_1$}}%
         {\textstyle\raise.4ex\hbox{$\textstyle\tilde\chi^-_1$}}%
       {\scriptstyle\raise.3ex\hbox{$\scriptstyle\tilde\chi^-_1$}}%
 {\scriptscriptstyle\raise.3ex\hbox{$\scriptscriptstyle\tilde\chi^-_1$}}}\xspace}
\newcommand*{\chinoonepm}{\ensuremath{\mathchoice%
      {\displaystyle\raise.4ex\hbox{$\displaystyle\tilde\chi^\pm_1$}}%
         {\textstyle\raise.4ex\hbox{$\textstyle\tilde\chi^\pm_1$}}%
       {\scriptstyle\raise.3ex\hbox{$\scriptstyle\tilde\chi^\pm_1$}}%
 {\scriptscriptstyle\raise.3ex\hbox{$\scriptscriptstyle\tilde\chi^\pm_1$}}}\xspace}

\newcommand*{\chinotwop}{\ensuremath{\mathchoice%
      {\displaystyle\raise.4ex\hbox{$\displaystyle\tilde\chi^+_2$}}%
         {\textstyle\raise.4ex\hbox{$\textstyle\tilde\chi^+_2$}}%
       {\scriptstyle\raise.3ex\hbox{$\scriptstyle\tilde\chi^+_2$}}%
 {\scriptscriptstyle\raise.3ex\hbox{$\scriptscriptstyle\tilde\chi^+_2$}}}\xspace}
\newcommand*{\chinotwom}{\ensuremath{\mathchoice%
      {\displaystyle\raise.4ex\hbox{$\displaystyle\tilde\chi^-_2$}}%
         {\textstyle\raise.4ex\hbox{$\textstyle\tilde\chi^-_2$}}%
       {\scriptstyle\raise.3ex\hbox{$\scriptstyle\tilde\chi^-_2$}}%
 {\scriptscriptstyle\raise.3ex\hbox{$\scriptscriptstyle\tilde\chi^-_2$}}}\xspace}
\newcommand*{\chinotwopm}{\ensuremath{\mathchoice%
      {\displaystyle\raise.4ex\hbox{$\displaystyle\tilde\chi^\pm_2$}}%
         {\textstyle\raise.4ex\hbox{$\textstyle\tilde\chi^\pm_2$}}%
       {\scriptstyle\raise.3ex\hbox{$\scriptstyle\tilde\chi^\pm_2$}}%
 {\scriptscriptstyle\raise.3ex\hbox{$\scriptscriptstyle\tilde\chi^\pm_2$}}}\xspace}

\newcommand*{\nino}{\ensuremath{\mathchoice%
      {\displaystyle\raise.4ex\hbox{$\displaystyle\tilde\chi^0$}}%
         {\textstyle\raise.4ex\hbox{$\textstyle\tilde\chi^0$}}%
       {\scriptstyle\raise.3ex\hbox{$\scriptstyle\tilde\chi^0$}}%
 {\scriptscriptstyle\raise.3ex\hbox{$\scriptscriptstyle\tilde\chi^0$}}}\xspace}

\newcommand*{\ninoone}{\ensuremath{\mathchoice%
      {\displaystyle\raise.4ex\hbox{$\displaystyle\tilde\chi^0_1$}}%
         {\textstyle\raise.4ex\hbox{$\textstyle\tilde\chi^0_1$}}%
       {\scriptstyle\raise.3ex\hbox{$\scriptstyle\tilde\chi^0_1$}}%
 {\scriptscriptstyle\raise.3ex\hbox{$\scriptscriptstyle\tilde\chi^0_1$}}}\xspace}
\newcommand*{\ninotwo}{\ensuremath{\mathchoice%
      {\displaystyle\raise.4ex\hbox{$\displaystyle\tilde\chi^0_2$}}%
         {\textstyle\raise.4ex\hbox{$\textstyle\tilde\chi^0_2$}}%
       {\scriptstyle\raise.3ex\hbox{$\scriptstyle\tilde\chi^0_2$}}%
 {\scriptscriptstyle\raise.3ex\hbox{$\scriptscriptstyle\tilde\chi^0_2$}}}\xspace}
\newcommand*{\ninothree}{\ensuremath{\mathchoice%
      {\displaystyle\raise.4ex\hbox{$\displaystyle\tilde\chi^0_3$}}%
         {\textstyle\raise.4ex\hbox{$\textstyle\tilde\chi^0_3$}}%
       {\scriptstyle\raise.3ex\hbox{$\scriptstyle\tilde\chi^0_3$}}%
 {\scriptscriptstyle\raise.3ex\hbox{$\scriptscriptstyle\tilde\chi^0_3$}}}\xspace}
\newcommand*{\ninofour}{\ensuremath{\mathchoice%
      {\displaystyle\raise.4ex\hbox{$\displaystyle\tilde\chi^0_4$}}%
         {\textstyle\raise.4ex\hbox{$\textstyle\tilde\chi^0_4$}}%
       {\scriptstyle\raise.3ex\hbox{$\scriptstyle\tilde\chi^0_4$}}%
 {\scriptscriptstyle\raise.3ex\hbox{$\scriptscriptstyle\tilde\chi^0_4$}}}\xspace}

\newcommand*{\gravino   }{\ensuremath{\tilde{G}}\xspace}
\newcommand*{\Zprime    }{\ensuremath{Z^\prime}\xspace}
\newcommand*{\Zstar     }{\ensuremath{Z^{*}}\xspace}
\newcommand*{\squark    }{\ensuremath{\tilde{q}}\xspace}
\newcommand*{\squarkL   }{\ensuremath{\tilde{q}_{\mathrm{L}}}\xspace}
\newcommand*{\squarkR   }{\ensuremath{\tilde{q}_{\mathrm{R}}}\xspace}
\newcommand*{\gluino    }{\ensuremath{\tilde{g}}\xspace}
\renewcommand*{\stop    }{\ensuremath{\tilde{t}}\xspace}
\newcommand*{\stopone   }{\ensuremath{\tilde{t}_1}\xspace}
\newcommand*{\stoptwo   }{\ensuremath{\tilde{t}_2}\xspace}
\newcommand*{\stopL     }{\ensuremath{\tilde{t}_{\mathrm{L}}}\xspace}
\newcommand*{\stopR     }{\ensuremath{\tilde{t}_{\mathrm{R}}}\xspace}
\newcommand*{\sbottom   }{\ensuremath{\tilde{b}}\xspace}
\newcommand*{\sbottomone}{\ensuremath{\tilde{b}_1}\xspace}
\newcommand*{\sbottomtwo}{\ensuremath{\tilde{b}_2}\xspace}
\newcommand*{\sbottomL  }{\ensuremath{\tilde{b}_{\mathrm{L}}}\xspace}
\newcommand*{\sbottomR  } {\ensuremath{\tilde{b}_{\mathrm{R}}}\xspace}
\newcommand*{\slepton   }{\ensuremath{\tilde{\ell}}\xspace}
\newcommand*{\sleptonL  }{\ensuremath{\tilde{\ell}_{\mathrm{L}}}\xspace}
\newcommand*{\sleptonR  }{\ensuremath{\tilde{\ell}_{\mathrm{R}}}\xspace}
\newcommand*{\sel       }{\ensuremath{\tilde{e}}\xspace}
\newcommand*{\selL      }{\ensuremath{\tilde{e}_{\mathrm{L}}}\xspace}
\newcommand*{\selR      }{\ensuremath{\tilde{e}_{\mathrm{R}}}\xspace}
\newcommand*{\smu       }{\ensuremath{\tilde{\mu}}\xspace}
\newcommand*{\smuL      }{\ensuremath{\tilde{\mu}_{\mathrm{L}}}\xspace}
\newcommand*{\smuR      }{\ensuremath{\tilde{\mu}_{\mathrm{R}}}\xspace}
\newcommand*{\stau      }{\ensuremath{\tilde{\tau}}\xspace}
\newcommand*{\stauL     }{\ensuremath{\tilde{\tau}_{\mathrm{L}}}\xspace}
\newcommand*{\stauR     }{\ensuremath{\tilde{\tau}_{\mathrm{R}}}\xspace}
\newcommand*{\stauone   }{\ensuremath{\tilde{\tau}_1}\xspace}
\newcommand*{\stautwo   }{\ensuremath{\tilde{\tau}_2}\xspace}
\newcommand*{\snu       }{\ensuremath{\tilde{\nu}}\xspace}

% +--------------------------------------------------------------------+
% | Masses                                                             |
% +--------------------------------------------------------------------+
\newcommand*{\mh}{\ensuremath{m_{h}}\xspace}
\newcommand*{\mW}{\ensuremath{m_{W}}\xspace}
\newcommand*{\mZ}{\ensuremath{m_{Z}}\xspace}
\newcommand*{\mH}{\ensuremath{m_{H}}\xspace}

% +--------------------------------------------------------------------+
% |  Useful things for proton-proton physics                           |
% +--------------------------------------------------------------------+
\newcommand*{\pT  }{\ensuremath{p_{\text{T}}}\xspace}
\newcommand*{\pt  }{\ensuremath{p_{\text{T}}}\xspace}
\newcommand*{\ET  }{\ensuremath{E_{\text{T}}}\xspace}
\newcommand*{\eT  }{\ensuremath{E_{\text{T}}}\xspace}
\newcommand*{\et  }{\ensuremath{E_{\text{T}}}\xspace}
\newcommand*{\HT  }{\ensuremath{H_{\text{T}}}\xspace}
\newcommand*{\pTsq}{\ensuremath{p_{\text{T}}^{2}}\xspace}
\newcommand*{\MET }{\ensuremath{E_{\text{T}}^{\text{miss}}}\xspace}
\newcommand*{\met }{\ensuremath{E_{\text{T}}^{\text{miss}}}\xspace}
\newcommand*{\Ecm }{\ensuremath{E_{\text{cm}}}\xspace}
\newcommand*{\rts }{\ensuremath{\sqrt{s}}\xspace}
\newcommand*{\sqs }{\ensuremath{\sqrt{s}}\xspace}

% +--------------------------------------------------------------------+
% |  Monte Carlo generators                                            |
% +--------------------------------------------------------------------+
\newcommand*{\ACERMC    }{\textsc{AcerMC}\xspace}
\newcommand*{\ACERMCV   }[1]{\textsc{AcerMC}~#1\xspace}
\newcommand*{\ALPGEN    }{\textsc{Alpgen}\xspace}
\newcommand*{\ALPGENV   }[1]{\textsc{Alpgen}~#1\xspace}
\newcommand*{\GEANT     }{\textsc{Geant}\xspace}
\newcommand*{\Herwigpp  }{Herwig++\xspace}
\newcommand*{\HERWIGpp  }{Herwig++\xspace}
\newcommand*{\Herwig    }{Herwig\xspace}
\newcommand*{\HerwigV   }[1]{Herwig~#1\xspace}
\newcommand*{\HERWIG    }{\textsc{Herwig}\xspace}
\newcommand*{\HERWIGV   }[1]{\textsc{Herwig}~#1\xspace}
\newcommand*{\JIMMY     }{\textsc{Jimmy}\xspace}
\newcommand*{\JIMMYV    }[1]{\textsc{Jimmy}~#1\xspace}
\newcommand*{\MADSPIN   }{\textsc{MadSpin}\xspace}
\newcommand*{\MADGRAPH  }{\textsc{MadGraph}\xspace}
\newcommand*{\MADGRAPHV }[1]{\textsc{MadGraph}~#1\xspace}
\newcommand*{\MGMCatNLO }{\textsc{MadGraph5}\_aMC@NLO\xspace} 
\newcommand*{\MGMCatNLOV}[1]{\textsc{MadGraph5}\_aMC@NLO~#1\xspace} 
\newcommand*{\MCatNLO   }{MC@NLO\xspace}
\newcommand*{\MCatNLOV  }[1]{MC@NLO~#1\xspace}
\newcommand*{\AMCatNLO  }{aMC@NLO\xspace}
\newcommand*{\AMCatNLOV }[1]{aMC@NLO~#1\xspace}
\newcommand*{\MCFM      }{MCFM\xspace}
\newcommand*{\MCFMV     }[1]{MCFM~#1\xspace}
\newcommand*{\METOP     }{\textsc{MEtop}\xspace}
\newcommand*{\METOPV    }[1]{\textsc{MEtop}~#1\xspace}
\newcommand*{\POWHEG    }{\textsc{Powheg}\xspace}
\newcommand*{\POWHEGV   }[1]{\textsc{Powheg}~#1\xspace}
\newcommand*{\POWHEGBOX }{\textsc{Powheg-Box}\xspace}
\newcommand*{\POWHEGBOXV}[1]{\textsc{Powheg-Box}~#1\xspace}
\newcommand*{\POWPYTHIA }{\POWHEG{}+\PYTHIA}
\newcommand*{\PROTOS    }{\textsc{Protos}\xspace}
\newcommand*{\PYTHIA    }{\textsc{Pythia}\xspace}
\newcommand*{\PYTHIAV   }[1]{\textsc{Pythia}~#1\xspace}
\newcommand*{\SHERPA    }{\textsc{Sherpa}\xspace}
\newcommand*{\SHERPAV   }[1]{\textsc{Sherpa}~#1\xspace}

% Event generator extras
\newcommand*{\Comphep }{CompHEP\xspace}
\newcommand*{\Prospino}{Prospino\xspace}

\newcommand*{\LO}{\ensuremath{\text{LO}}\xspace}
\newcommand*{\NLO}{\ensuremath{\text{NLO}}\xspace}
\newcommand*{\NLL}{\ensuremath{\text{NLL}}\xspace}
\newcommand*{\NNLO}{\ensuremath{\text{N}}\NLO\xspace}
\newcommand*{\muF}{\ensuremath{\mu_\textsc{f}}\xspace}
\newcommand*{\muR}{\ensuremath{\mu_\textsc{r}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%journal.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%These are the macros for inputting journal, conferences, and books.
%They are used by the Sports Section and the Minireviews
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Reference abbreviations
%Example:  \nim212,319(1983)
%
%Reference abbreviations
%Example:  \nim212,319(1983)
\def\anp#1,#2(#3){{\rm Adv.\ Nucl.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\aip#1,#2(#3){{\rm Am.\ Inst.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\aj#1,#2(#3){{\rm Astrophys.\ J.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\ajs#1,#2(#3){{\rm Astrophys.\ J.\ Supp.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\ajl#1,#2(#3){{\rm Astrophys.\ J.\ Lett.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\ajp#1,#2(#3){{\rm Am.\ J.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\apny#1,#2(#3){{\rm Ann.\ Phys.\ (NY)\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\apnyB#1,#2(#3){{\rm Ann.\ Phys.\ (NY)\ }{\bf B#1}, {\rm#2} {\rm(#3)}}
\def\apD#1,#2(#3){{\rm Ann.\ Phys.\ }{\bf D#1}, {\rm#2} {\rm(#3)}}
\def\ap#1,#2(#3){{\rm Ann.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\apl#1,#2(#3){{\rm Appl.\ Phys.\ Lett.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\ass#1,#2(#3){{\rm Ap.\ Space Sci.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\astropp#1,#2(#3){{\rm Astropart.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\aap#1,#2(#3){{\rm Astron.\ \& Astrophys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\araa#1,#2(#3){{\rm Ann.\ Rev.\ Astron.\ Astrophys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\arnps#1,#2(#3){{\rm Ann.\ Rev.\ Nucl.\ and Part.\ Sci.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\arns#1,#2(#3){{\rm Ann.\ Rev.\ Nucl.\ Sci.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\cpc#1,#2(#3){{\rm Comp.\ Phys.\ Comm.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\cpC#1,#2(#3){{\rm Chin.\ Phys.\ C\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\cjp#1,#2(#3){{\rm Can.\ J.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\cmp#1,#2(#3){{\rm Commun.\ Math.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\cnpp#1,#2(#3){{\rm Comm.\ Nucl.\ Part.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\cnppA#1,#2(#3){{\rm Comm.\ Nucl.\ Part.\ Phys.\ }{\bf A#1}, {\rm#2} {\rm(#3)}}
\def\cqg#1,#2(#3){{\rm Class.\ Quantum Grav.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\epj#1,#2(#3){{\rm Eur.\ Phys.\ J.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\epjA#1,#2(#3){{\rm Eur.\ Phys.\ J.\ }{\bf A#1}, {\rm#2} {\rm(#3)}}
\def\epjC#1,#2(#3){{\rm Eur.\ Phys.\ J.\ }{\bf C#1}, {\rm#2} {\rm(#3)}}
\def\epjH#1,#2(#3){{\rm Eur.\ Phys.\ J.\ }{\bf H#1}, {\rm#2} {\rm(#3)}}
\def\el#1,#2(#3){{\rm Europhys.\ Lett.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\grg#1,#2(#3){{\rm Gen.\ Rel.\ Grav.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\hpa#1,#2(#3){{\rm Helv.\ Phys.\ Acta\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\ieeetNS#1,#2(#3){{\rm IEEE Trans.\ }{\bf NS#1}, {\rm#2} {\rm(#3)}}
\def\IEEE #1,#2(#3){{\rm IEEE\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\ijar#1,#2(#3){{\rm Int.\ J.\ of Applied Rad.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\ijari#1,#2(#3){{\rm Int.\ J.\ of Applied Rad.\ and Isotopes\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\jcap#1,#2(#3){{\rm JCAP\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\jcp#1,#2(#3){{\rm J.\ Chem.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\jgr#1,#2(#3){{\rm J.\ Geophys.\ Res.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\jetp#1,#2(#3){{\rm Sov.\ Phys.\ JETP\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\jetpl#1,#2(#3){{\rm Sov.\ Phys.\ JETP Lett.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\jhep#1,#2(#3){{\rm JHEP\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\jmp#1,#2(#3){{\rm J.\ Math.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\jpA#1,#2(#3){{\rm J.\ Phys.\ }{\bf A#1}, {\rm#2} {\rm(#3)}}
\def\jpG#1,#2(#3){{\rm J.\ Phys.\ }{\bf G#1}, {\rm#2} {\rm(#3)}}
\def\jpamg#1,#2(#3){{\rm J.\ Phys.\ A: Math.\ and Gen.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\jpcrd#1,#2(#3){{\rm J.\ Phys.\ Chem.\ Ref.\ Data\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\jpsj#1,#2(#3){{\rm J.\ Phys.\ Soc.\ Jpn.\ }{\bf G#1}, {\rm#2} {\rm(#3)}}
\def\lnc#1,#2(#3){{\rm Lett.\ Nuovo Cimento\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\nature#1,#2(#3){{\rm Nature\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\natp#1,#2(#3){{\rm Nat. Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\nc#1,#2(#3){{\rm Nuovo Cimento\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\nim#1,#2(#3){{\rm Nucl.\ Instrum.\ Methods\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\nimA#1,#2(#3){{\rm Nucl.\ Instrum.\ Methods\ }{\bf A#1}, {\rm#2} {\rm(#3)}}
\def\nimB#1,#2(#3){{\rm Nucl.\ Instrum.\ Methods\ }{\bf B#1}, {\rm#2} {\rm(#3)}}
\def\np#1,#2(#3){{\rm Nucl.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\mnras#1,#2(#3){{\rm Mon.\ Not.\ R.\ Astron.\ Soc\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\medp#1,#2(#3){{\rm Med.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\mplA#1,#2(#3){{\rm Mod.\ Phys.\ Lett.\ }{\bf A#1}, {\rm#2} {\rm(#3)}}
\def\njp#1,#2(#3){{\rm New\ J.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\npA#1,#2(#3){{\rm Nucl.\ Phys.\ }{\bf A#1}, {\rm#2} {\rm(#3)}}
\def\npB#1,#2(#3){{\rm Nucl.\ Phys.\ }{\bf B#1}, {\rm#2} {\rm(#3)}}
\def\npBps#1,#2(#3){{\rm Nucl.\ Phys.\ (Proc.\ Supp.)\ }{\bf B#1}, {\rm#2} {\rm(#3)}}
\def\npps#1,#2(#3){{\rm Nucl.\ Phys.\ (Proc.\ Supp.)\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\pasp#1,#2(#3){{\rm Pub.\ Astron.\ Soc.\ Pac.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\pl#1,#2(#3){{\rm Phys.\ Lett.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\fp#1,#2(#3){{\rm Fortsch.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\ijmpA#1,#2(#3){{\rm Int.\ J.\ Mod.\ Phys.\ }{\bf A#1}, {\rm#2} {\rm(#3)}}
\def\ijmpD#1,#2(#3){{\rm Int.\ J.\ Mod.\ Phys.\ }{\bf D#1}, {\rm#2} {\rm(#3)}}
\def\ijmpE#1,#2(#3){{\rm Int.\ J.\ Mod.\ Phys.\ }{\bf E#1}, {\rm#2} {\rm(#3)}}
\def\plA#1,#2(#3){{\rm Phys.\ Lett.\ }{\bf A#1}, {\rm#2} {\rm(#3)}}
\def\plB#1,#2(#3){{\rm Phys.\ Lett.\ }{\bf B#1}, {\rm#2} {\rm(#3)}}
\def\pnasus#1,#2(#3){{\it Proc.\ Natl.\ Acad.\ Sci.\ \rm (US)}{B#1}, {\rm#2} {\rm(#3)}}
\def\ppsA#1,#2(#3){{\rm Proc.\ Phys.\ Soc.\ }{\bf A#1}, {\rm#2} {\rm(#3)}}
\def\ppsB#1,#2(#3){{\rm Proc.\ Phys.\ Soc.\ }{\bf B#1}, {\rm#2} {\rm(#3)}}
\def\pr#1,#2(#3){{\rm Phys.\ Rev.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\prA#1,#2(#3){{\rm Phys.\ Rev.\ }{\bf A#1}, {\rm#2} {\rm(#3)}}
\def\prB#1,#2(#3){{\rm Phys.\ Rev.\ }{\bf B#1}, {\rm#2} {\rm(#3)}}
\def\prC#1,#2(#3){{\rm Phys.\ Rev.\ }{\bf C#1}, {\rm#2} {\rm(#3)}}
\def\prD#1,#2(#3){{\rm Phys.\ Rev.\ }{\bf D#1}, {\rm#2} {\rm(#3)}}
\def\prX#1,#2(#3){{\rm Phys.\ Rev.\ }{\bf X#1}, {\rm#2} {\rm(#3)}}
\def\prab#1,#2(#3){{\rm Phys.\ Rev.\ Accel. Beams\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\prept#1,#2(#3){{\rm Phys.\ Reports\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\preptC#1,#2(#3){{\rm Phys.\ Reports\ }{\bf C#1}, {\rm#2} {\rm(#3)}}
\def\prslA#1,#2(#3){{\rm Proc.\ Royal Soc.\ London\ }{\bf A#1}, {\rm#2} {\rm(#3)}}
\def\prl#1,#2(#3){{\rm Phys.\ Rev.\ Lett.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\ps#1,#2(#3){{\rm Phys.\ Scripta\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\ptp#1,#2(#3){{\rm Prog.\ Theor.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\ptep#1,#2(#3){{\rm Prog.\ Theor.\ Exp.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\ppn#1,#2(#3){{\rm Phys.\ of Part.\ and\ Nucl.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\ppnp#1,#2(#3){{\rm Prog.\ in Part.\ Nucl.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\ptps#1,#2(#3){{\rm Prog.\ Theor.\ Phys.\ Supp.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\pw#1,#2(#3){{\rm Part.\ World\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\pzetf#1,#2(#3){{\rm Pisma Zh.\ Eksp.\ Teor.\ Fiz.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\rgss#1,#2(#3){{\rm Revs.\ Geophysics \& Space Sci.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\rmp#1,#2(#3){{\rm Rev.\ Mod.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\rnc#1,#2(#3){{\rm Riv.\ Nuovo Cimento\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\rpp#1,#2(#3){{\rm Rept.\ on Prog.\ in Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\science#1,#2(#3){{\rm Science\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\sjnp#1,#2(#3){{\rm Sov.\ J.\ Nucl.\ Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\sjpn#1,#2(#3){{\rm Sov.\ J.\ Part.\ Nucl.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\panp#1,#2(#3){{\rm Phys.\ Atom.\ Nucl.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\spu#1,#2(#3){{\rm Sov.\ Phys.\ Usp.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\surveyHEP#1,#2(#3){{\rm Surv.\ High Energy Physics\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\yf#1,#2(#3){{\rm Yad.\ Fiz.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\zetf#1,#2(#3){{\rm Zh.\ Eksp.\ Teor.\ Fiz.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\zp#1,#2(#3){{\rm Z.~Phys.\ }{\bf #1}, {\rm#2} {\rm(#3)}}
\def\zpA#1,#2(#3){{\rm Z.~Phys.\ }{\bf A#1}, {\rm#2} {\rm(#3)}}
\def\zpC#1,#2(#3){{\rm Z.~Phys.\ }{\bf C#1}, {\rm#2} {\rm(#3)}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

